Future physics opportunities for high-density QCD at the LHC with heavy-ion and proton beams

The future opportunities for high-density QCD studies with ion and proton beams at the LHC are presented. Four major scientific goals are identified: the characterisation of the macroscopic long wavelength Quark-Gluon Plasma (QGP) properties with unprecedented precision, the investigation of the microscopic parton dynamics underlying QGP properties, the development of a unified picture of particle production and QCD dynamics from small (pp) to large (nucleus--nucleus) systems, the exploration of parton densities in nuclei in a broad ($x$, $Q^2$) kinematic range and the search for the possible onset of parton saturation. In order to address these scientific goals, high-luminosity Pb-Pb and p-Pb programmes are considered as priorities for Runs 3 and 4, complemented by high-multiplicity studies in pp collisions and a short run with oxygen ions. High-luminosity runs with intermediate-mass nuclei, for example Ar or Kr, are considered as an appealing case for extending the heavy-ion programme at the LHC beyond Run 4. The potential of the High-Energy LHC to probe QCD matter with newly-available observables, at twice larger center-of-mass energies than the LHC, is investigated.

==> accelerator/Run1Run2Table.tex <==
%% Complete table with Pb-Pb and p-Pb but it is too wide for the page
%% This is not used in the document now but keep the file for possible future use.
{\renewcommand{\arraystretch}{1.4}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\footnotesize
\begin{tabular}{L{2.1cm}|cc|cccccc|c@{}}
\hline                   
  Quantity                        & \multicolumn{2}{c|}{``design''} & \multicolumn{6}{c|}{achieved} & upgrade \\
  \hline
Year                                & (2004)&(2011)  & 2010 & 2011 &2012--13& 2015 &2016& 2018 $\ge$2021 \\
Weeks in physics & - & - & 4 & 3.5& 3 & 2.5& 1, 2 & 3.5 &-\\
Fill no. (best)  & & & 1541 & 2351 & 3544& 4720 &5562&7473& -\\
%circumference $C$   & km            & \multicolumn{5}{c}{ 26.659 } \\
%%mass and charge numbers $A,Z$   & ...  & \multicolumn{3}{c}{--- 208, 82 ---} \\
Species                         &\PbPb &\textcolor{red}{\pPb}& \PbPb&\PbPb & \textcolor{red}{\pPb}& \PbPb &\textcolor{red}{\pPb} &\PbPb& \PbPb \\
Beam energy \qty{E[Z}{TeV]}  & \multicolumn{2}{c|}{ 7 } & \multicolumn{2}{c}{3.5} & 4 & 6.37  & 4,6.5 & 6.37 & 7 \\
Pb beam energy \qty{E[A}{ TeV]}  & \multicolumn{2}{c|}{2.76} & \multicolumn{2}{c}{ 1.38 } & 1.58 &   2.51 & 1.58,2.56 &2.51 & 2.76 \\
\raggedright Collision energy \qty{\sqrt{\sNN}}{[TeV]}  & 5.52& \textcolor{red}{8.79}& \multicolumn{2}{c}{2.51}& \textcolor{red}{\textbf{5.02}} & \textbf{5.02}& \textcolor{red}{\textbf{5.02},8.16}&\textcolor{red}{\textbf{5.02}} & 5.52  \\
\hline
Bunch intensity \qty{N_b}{[10^8]}       & \multicolumn{2}{c|}{0.7} & 1.22 &1.07   & 1.2 & 2.0 &2.1&2.2 &1.8 \\
No. \ of bunches $k_b$             & 592& &137& 338  & 358  & 518 & 540 &733 &1232 \\
%%Colliding bunches  $k_c$             & 592& & &    &   &  & 912\\
Pb norm. emittance \qty{\epsilon_N}{[\mu m]}  & \multicolumn{2}{c|}{ 1.5 }  & 2.& 2.0 & 2. & 2.1 & 1.6 &2.0&   1.65   \\
Pb bunch length \qty{\sigma_{z}}{m}   & \multicolumn{2}{c|}{0.08} & \multicolumn{6}{c|}{0.07--0.1} &  0.08 \\
\qty{\bstar}{[m]}&       \multicolumn{2}{c|}{0.5}& 3.5 & 1.0 & 0.8 & 0.8  & 10, 0.6 &0.5 &0.5\\
%beam-beam parameter $\xi$/IP  $10^{-3}$   & 0.20 & 0.35 &   &  & 0.64 \\
Pb stored energy   MJ/beam    & 3.8 & 2.3 &0.65   & 1.9 &  2.77 & 8.6  & 9.7 &13.3&  21 \\
\hline
Luminosity \qty{\LAA}{[10^{27}cm^{-2}s^{-1}]}   & 1& \textcolor{red}{150} &0.03  & 0.5  & \textcolor{red}{116}  & 3.6  &\textcolor{red}{850}&\textcolor{red}{6.1}& 7   \\
NN luminosity \qty{ \LNN}{[10^{30} {cm}^{-2} {s}^{-1}]}   &\fbox{43}   & \fbox{31}   & 1.3  & 22. & 24& 156 & \fbox{177}&\fbox{264}& \fbox{303}  \\
Integrated luminosity/experiment [\qty{}{\mu b^{-1}}]& 1000 & \textcolor{red}{$10^5$}  &  9  & 160 & \textcolor{red}{32000} & 433,585 &\textcolor{red}{\enum{1.9}{5}} &\textcolor{red}{900,1800} & $10^4$ \\
%Int. NN lumi./expt. [\qty{}{nb^{-1}}]& \enum{4.3}{4} & \enum{2.1}{4}  &  ~380  & ~6700 & 6650 & \enum{2.8}{4} &\enum{4.0}{4} & \enum{4.3}{5} \\
Int. NN lumi./expt. [\qty{}{pb^{-1}}]& 43 & 21  &  ~0.38  & ~6.7 & 6.7 & 19,25.3& 40&39,80 & \enum{4.3}{5} \\
 \hline
\end{tabular}
}
 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This is a commented out backup copy of above before adding 2018 column 
\iffalse 
{\renewcommand{\arraystretch}{1.2}
\begin{tabular}{m{3.7cm}|cc|ccccc|c@{}}
\hline                   
  Quantity                        & \multicolumn{2}{c|}{``design''} & \multicolumn{5}{c|}{achieved} & upgrade \\
  \hline
Year                                & (2004)&(2011)  & 2010 & 2011 &2012--13& 2015 &2016& $\ge$2021 \\
Weeks in physics & - & - & 4 & 3.5& 3 & 2.5& 1, 2 &-\\
Fill no. (best)  & & & 1541 & 2351 & 3544& 4720 &5562& -\\
%circumference $C$   & km            & \multicolumn{5}{c}{ 26.659 } \\
%%mass and charge numbers $A,Z$   & ...  & \multicolumn{3}{c}{--- 208, 82 ---} \\
Species                         &\PbPb &\textcolor{red}{\pPb}& \PbPb&\PbPb & \textcolor{red}{\pPb}& \PbPb &\textcolor{red}{\pPb}& \PbPb \\
Beam energy \qty{E[Z}{TeV]}  & \multicolumn{2}{c|}{ 7 } & \multicolumn{2}{c}{3.5} & 4 & 6.37  & 4,6.5 & 7 \\
Pb beam energy \qty{E[A}{ TeV]}  & \multicolumn{2}{c|}{2.76} & \multicolumn{2}{c}{ 1.38 } & 1.58 &   2.51 & 1.58,2.56  & 2.76 \\
\raggedright Collision energy \qty{\sqrt{\sNN}}{[TeV]}  & 5.52& \textcolor{red}{8.79}& \multicolumn{2}{c}{2.51}& \textcolor{red}{\textbf{5.02}} & \textbf{5.02}& \textcolor{red}{\textbf{5.02},8.16}& 5.52  \\
\hline
Bunch intensity \qty{N_b}{[10^8]}       & \multicolumn{2}{c|}{0.7} & 1.22 &1.07   & 1.2 & 2.0 &2.1 &1.8 \\
No,\ of bunches $k_b$             & 592& &137& 338  & 358  & 518 & 540 &1232 \\
%%Colliding bunches  $k_c$             & 592& & &    &   &  & 912\\
Pb norm. emittance \qty{\epsilon_N}{[\mu m]}  & \multicolumn{2}{c|}{ 1.5 }  & 2.& 2.0 & 2. & 2.1 & 1.6 &  1.65   \\
Pb bunch length \qty{\sigma_{z}}{m}   & \multicolumn{2}{c|}{0.08} & \multicolumn{5}{c|}{0.07--0.1} &  0.08 \\
\qty{\bstar}{[m]}&       \multicolumn{2}{c|}{0.5}& 3.5 & 1.0 & 0.8 & 0.8  & 10, 0.6  &0.5\\
%beam-beam parameter $\xi$/IP  $10^{-3}$   & 0.20 & 0.35 &   &  & 0.64 \\
Pb stored energy   MJ/beam    & 3.8 & 2.3 &0.65   & 1.9 &  2.77 & 8.6  & 9.7 &  21 \\
\hline
Luminosity \qty{\LAA}{[10^{27}cm^{-2}s^{-1}]}   & 1& \textcolor{red}{150} &0.03  & 0.5  & \textcolor{red}{116}  & 3.6  &\textcolor{red}{850}& 6   \\
NN luminosity \qty{ \LNN}{[10^{30} {cm}^{-2} {s}^{-1}]}   &\fbox{43}   & \fbox{31}   & 1.3  & 22. & 24& \fbox{156} & \fbox{177}& \fbox{260}  \\
Integrated luminosity/experiment [\qty{}{\mu b^{-1}}]& 1000 & \textcolor{red}{$10^5$}  &  9  & 160 & \textcolor{red}{32000} & 650 &\textcolor{red}{\enum{1.9}{5}} & $10^4$ \\
%Int. NN lumi./expt. [\qty{}{nb^{-1}}]& \enum{4.3}{4} & \enum{2.1}{4}  &  ~380  & ~6700 & 6650 & \enum{2.8}{4} &\enum{4.0}{4} & \enum{4.3}{5} \\
Int. NN lumi./expt. [\qty{}{nb^{-1}}]& 43000 & 21000  &  ~380  & ~6700 & 6650 & 28000& 40000 & \enum{4.3}{5} \\
 \hline
\end{tabular}
}

\fi 


==> hf/authors.tex <==
\author{Conveners: E. Bruna$^{1}$, G.M. Innocenti$^{2,3}$ \\
Contributors: J. Aichelin$^{17}$, S. A. Bass$^{15}$, C. Bedda$^{6}$, A. Beraudo$^{1}$, G.E. Bruno$^{7}$, Z. Citron$^{13}$, A. Dainese$^{8}$, A. Dubla$^{9}$, F. Fionda$^{10}$, P.-B. Gossiaux$^{17}$, V. Greco$^{14}$, F. Grosa$^{11}$, Y.-J. Lee$^{3}$, J. Margutti$^{6}$, A. Mischke$^{6}$, S. Mohapatra$^{18}$, M. Peters$^{3}$, S. Plumari$^{14}$, F. Prino$^{1}$, A. Rossi$^{8}$, J. Sun$^{4}$,C. Terrevoli$^{8}$, B. Trzeciak$^{6}$, A. Uras$^{12}$, L. Van Doremalen$^{6}$, I. Vitev$^{16}$, J. Wang$^{3}$, T.-W. Wang$^{3}$, M. Winn$^{5}$,Y. Xu$^{15}$}
\institute{
$^{1}$ Universit\`a degli Studi di Torino and INFN, Italy \\
$^{2}$ European Organization for Nuclear Research (CERN), Geneva, Switzerland \\
$^{3}$ Massachusetts Institute of Technology (MIT), Cambridge, USA \\
$^{4}$ Tsinghua University, Beijing, China \\
$^{5}$ LAL, CNRS/IN2P3, Universit\'e Paris-Sud, Universit\'e Paris-Saclay, 
Orsay, France  and IRFU/DPhN, CEA Saclay, Universit\'e Paris-Saclay, Saclay, France 
 \\
$^{6}$ Utrecht University, Utrecht, the Netherlands \\
$^{7}$ Politecnico di Bari and INFN, Bary, Italy \\
$^{8}$ Universit\`a degli Studi di Padova and INFN, Padova, Italy \\
$^{9}$ GSI Helmholzzentrum f\"{u}r Schwerionenforschung, Darmstadt, Germany \\
$^{10}$ University of Bergen, Bergen, Norway \\
$^{11}$ Politecnico di Torino and INFN, Torino, Italy \\
$^{12}$ IPN-Lyon, Villeurbanne, France \\
$^{13}$ Ben-Gurion University of the Negev, Beersheba, Israel \\
$^{14}$ Universit\`a di Catania and INFN, Catania, Italy \\
$^{15}$ Duke University, Durham, USA \\
$^{16}$ Los Alamos National Laboratory, Los Alamos, USA \\
$^{17}$ SUBATECH, Nantes, France \\
$^{18}$ Columbia University, New York, USA \\
}




==> hf/conclusions.tex <==
\textbf{FIGURES}:
\begin{enumerate}
\item Summary figure with different Lint scenarios?
\end{enumerate}


==> jets/Conclusion.tex <==
\subsection{Summary}


==> jets/definitions.tex <==
\newcommand{\ptjet}        {\ensuremath{p_{\mathrm{T,jet}}}}
\newcommand{\gevc}         {\UGeVc}
\newcommand{\ptjetch}      {\ensuremath{p_{\mathrm{T,jet}}^{\mathrm{ch}}}}
\newcommand{\Dphi}         {\ensuremath{\Delta\varphi}}
\newcommand{\dphithresh}   {\ensuremath{\Delta\varphi_{\mathrm{thresh}}}}
\newcommand{\pythia}       {{\textsc{Pythia}}\xspace}
\newcommand{\jewel}        {{\textsc{Jewel}}\xspace}
\newcommand{\fastjet}      {{\textsc{FastJet}}\xspace}
\newcommand{\akt}          {\ensuremath{{\rm anti-}k_{\rm t}}}


==> lightflavour/summary.tex <==
\subsection{Summary}
\textcolor{blue}{Summary of experimental reach and sensitivity. Includes summary of section 2 and 3, outlook beyond HL-LHC. No figures foreseen.} 
